SIMQ: A Single Graph-based Index for Multi-Vector Query

Multi-vector retrieval models such as ColBERT achieve state-of-the-art effectiveness by representing documents as sets of token-level vectors and scoring via MaxSim, but their high computational cost limits scalability to large corpora. Existing approximate methods face fundamental bottlenecks: centroid interaction matrix approaches require computing a full matrix at every query and rely on GPU-accelerated clustering, while data-oblivious compression methods yield unstable recall that requires repeated compensation. We propose SIMQ (Single graph Index for Multi-vector Query), a framework that bridges single-vector graph indices and multi-vector retrieval through data-aware sampling-based clustering and per-token graph navigation, simultaneously bypassing all aforementioned bottlenecks. SIMQ organizes all token vectors into fine-grained clusters via data-aware sampling, builds a single graph index over cluster centroids independently of PLAID's residual representation, and approximates the MaxSim score through per-token graph search without materializing any interaction matrix or relying on GPU acceleration. We provide theoretical analysis showing that, under a manifold assumption and successful cell retrieval, data-aware partitioning has a smaller expected approximation error than a data-oblivious partition. Building on this foundation, SIMQ+ further introduces count-based scoring and a dynamic candidate set to improve robustness across varying query conditions. Experiments on five benchmarks compare recall, throughput, and construction time against several baselines, primarily on CPU; large-scale PLAID k-means centroids are built on a separate GPU machine. SIMQ has been integrated into VSAG, an Ant Group's open-source vector search library.

==> ack.tex <==
\section*{Acknowledgments}
\label{sec:ack}

This work was supported by [funding information to be added]. We thank the anonymous
reviewers for their constructive feedback.


==> figures/index_single_multi_compare.tex <==
\begin{tikzpicture}[x=1pt,y=1pt,baseline=(current bounding box.north)]
\definecolor{D62728}{HTML}{D62728}
\definecolor{1F77B4}{HTML}{1F77B4}
\definecolor{2CA02C}{HTML}{2CA02C}
\tikzset{imLine/.style={line width=1.45pt}, imGrid/.style={gray!55,dashed,line width=0.25pt}, imTick/.style={font=\small}}
\fill[white] (0,0) rectangle (350,335);
\draw[black,line width=0.45pt] (35,144) rectangle ++(142,92);
\draw[imGrid] (35.00,144) -- (35.00,236.00);
\node[anchor=north,imTick] at (35.00,141.00) {0.6};
\draw[imGrid] (80.00,144) -- (80.00,236.00);
\node[anchor=north,imTick] at (80.00,141.00) {0.7};
\draw[imGrid] (125.00,144) -- (125.00,236.00);
\node[anchor=north,imTick] at (125.00,141.00) {0.8};
\draw[imGrid] (170.00,144) -- (170.00,236.00);
\node[anchor=north,imTick] at (170.00,141.00) {0.9};
\draw[imGrid] (35,159.93) -- (177.00,159.93);
\draw[imGrid] (35,209.40) -- (177.00,209.40);
\node[anchor=east,imTick] at (32,161.93) {100};
\node[anchor=east,imTick] at (32,211.40) {200};
\node[rotate=90,anchor=south,imTick] at (13,190) {QPS};
\draw[D62728,imLine] (60.68,220.89) -- (92.62,218.47) -- (115.40,217.36) -- (128.17,216.82) -- (145.72,214.99) -- (155.36,214.59) -- (163.37,212.57) -- (163.81,212.72);
\fill[D62728] (60.68,220.89) circle (2.1pt);
\fill[D62728] (92.62,218.47) circle (2.1pt);
\fill[D62728] (115.40,217.36) circle (2.1pt);
\fill[D62728] (128.17,216.82) circle (2.1pt);
\fill[D62728] (145.72,214.99) circle (2.1pt);
\fill[D62728] (155.36,214.59) circle (2.1pt);
\fill[D62728] (163.37,212.57) circle (2.1pt);
\fill[D62728] (163.81,212.72) circle (2.1pt);
\draw[1F77B4,imLine] (93.48,217.12) -- (115.99,216.21) -- (129.48,215.64) -- (142.98,213.38) -- (151.98,211.91) -- (160.98,206.12) -- (165.48,199.25);
\fill[1F77B4] (93.48,219.12) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (115.99,218.21) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (129.48,217.64) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (142.98,215.38) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (151.98,213.91) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (160.98,208.12) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (165.48,201.25) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\draw[2CA02C,imLine] (75.49,214.50) -- (93.48,214.85) -- (102.48,214.43) -- (111.48,213.76) -- (129.48,211.84) -- (138.48,209.31) -- (142.98,204.88);
\fill[2CA02C] (75.49,216.50) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\fill[2CA02C] (93.48,216.85) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\fill[2CA02C] (102.48,216.43) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\fill[2CA02C] (111.48,215.76) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\fill[2CA02C] (129.48,213.84) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\fill[2CA02C] (138.48,211.31) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\fill[2CA02C] (142.98,206.88) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\draw[black,line width=0.45pt] (195,144) rectangle ++(142,92);
\draw[imGrid] (223.40,144) -- (223.40,236.00);
\node[anchor=north,imTick] at (223.40,141.00) {0.4};
\draw[imGrid] (251.80,144) -- (251.80,236.00);
\node[anchor=north,imTick] at (251.80,141.00) {0.5};
\draw[imGrid] (280.20,144) -- (280.20,236.00);
\node[anchor=north,imTick] at (280.20,141.00) {0.6};
\draw[imGrid] (308.60,144) -- (308.60,236.00);
\node[anchor=north,imTick] at (308.60,141.00) {0.7};
\draw[imGrid] (337.00,144) -- (337.00,236.00);
\node[anchor=north,imTick] at (337.00,141.00) {0.8};
\draw[imGrid] (195.00,144) -- (195.00,236.00);
\node[anchor=north,imTick] at (195.00,141.00) {0.3};
\draw[imGrid] (195,159.93) -- (337.00,159.93);
\draw[imGrid] (195,209.40) -- (337.00,209.40);
\draw[D62728,imLine] (213.88,227.54) -- (230.75,226.88) -- (255.90,225.28) -- (274.52,224.19) -- (284.52,223.60) -- (295.92,223.32) -- (308.16,221.81) -- (316.56,217.28) -- (323.09,211.68);
\fill[D62728] (213.88,227.54) circle (2.1pt);
\fill[D62728] (230.75,226.88) circle (2.1pt);
\fill[D62728] (255.90,225.28) circle (2.1pt);
\fill[D62728] (274.52,224.19) circle (2.1pt);
\fill[D62728] (284.52,223.60) circle (2.1pt);
\fill[D62728] (295.92,223.32) circle (2.1pt);
\fill[D62728] (308.16,221.81) circle (2.1pt);
\fill[D62728] (316.56,217.28) circle (2.1pt);
\fill[D62728] (323.09,211.68) circle (2.1pt);
\draw[1F77B4,imLine] (258.53,223.05) -- (275.57,221.37) -- (298.28,220.09) -- (309.63,210.36) -- (318.16,200.93) -- (320.99,194.15) -- (323.83,186.48);
\fill[1F77B4] (258.53,225.05) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (275.57,223.37) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (298.28,222.09) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (309.63,212.36) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (318.16,202.93) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (320.99,196.15) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (323.83,188.48) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\draw[2CA02C,imLine] (235.83,221.92) -- (264.21,217.94) -- (272.74,216.77) -- (295.44,208.36) -- (301.12,200.48) -- (306.79,192.70);
\fill[2CA02C] (235.83,223.92) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\fill[2CA02C] (264.21,219.94) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\fill[2CA02C] (272.74,218.77) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\fill[2CA02C] (295.44,210.36) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\fill[2CA02C] (301.12,202.48) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\fill[2CA02C] (306.79,194.70) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\node[anchor=north,font=\small] at (106,126) {Recall100@100};
\node[anchor=north,font=\small] at (266,126) {Recall100@100};
\node[rotate=90,anchor=south,fill=white,inner sep=1pt,imTick] at (201,190) {QPS};
\fill[D62728] (26,320) circle (2pt);
\node[anchor=west,font=\normalsize] at (33,316) {SIMQ(HNSW)};
\fill[1F77B4] (142,318) -- ++(3pt,0) -- ++(-1.5pt,3pt) -- cycle;
\node[anchor=west,font=\normalsize] at (151,316) {SIMQ(NSG)};
\fill[2CA02C] (258,320) -- ++(2pt,2pt) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- cycle;
\node[anchor=west,font=\normalsize] at (267,316) {SIMQ(DPG)};
\end{tikzpicture}


==> figures/pag_cluster_compare.tex <==
\begin{tikzpicture}[x=1pt,y=1pt,baseline=(current bounding box.north)]
\definecolor{D62728}{HTML}{D62728}
\definecolor{E69F00}{HTML}{E69F00}
\definecolor{7B61A8}{HTML}{7B61A8}
\tikzset{pcLine/.style={line width=1.25pt}, pcGrid/.style={gray!55,dashed,line width=0.3pt}, pcTick/.style={font=\small}}
\fill[white] (0,0) rectangle (700,360);
\draw[black,line width=0.5pt] (48,48) rectangle ++(315,220);
\draw[pcGrid] (57.62,48) -- (57.62,268);
\node[anchor=north,pcTick] at (57.62,44) {0.3};
\draw[pcGrid] (110.98,48) -- (110.98,268);
\node[anchor=north,pcTick] at (110.98,44) {0.4};
\draw[pcGrid] (164.33,48) -- (164.33,268);
\node[anchor=north,pcTick] at (164.33,44) {0.5};
\draw[pcGrid] (217.69,48) -- (217.69,268);
\node[anchor=north,pcTick] at (217.69,44) {0.6};
\draw[pcGrid] (271.05,48) -- (271.05,268);
\node[anchor=north,pcTick] at (271.05,44) {0.7};
\draw[pcGrid] (324.41,48) -- (324.41,268);
\node[anchor=north,pcTick] at (324.41,44) {0.8};
\node[anchor=south,font=\small\bfseries] at (205.5,277) {LoTTE};
\node[anchor=north,pcTick] at (205.5,24) {Recall@100};
\node[rotate=90,anchor=south,pcTick] at (18,158) {QPS};
\draw[D62728,pcLine] (242.72,189.79) -- (276.17,189.22) -- (293.35,188.64) -- (304.72,188.93) -- (326.49,188.06) -- (342.55,184.86) -- (346.13,178.39);
\fill[D62728] (242.72,189.79) circle (2.2pt);
\fill[D62728] (276.17,189.22) circle (2.2pt);
\fill[D62728] (293.35,188.64) circle (2.2pt);
\fill[D62728] (304.72,188.93) circle (2.2pt);
\fill[D62728] (326.49,188.06) circle (2.2pt);
\fill[D62728] (342.55,184.86) circle (2.2pt);
\fill[D62728] (346.13,178.39) circle (2.2pt);
\draw[E69F00,pcLine] (262.62,175.43) -- (287.96,175.43) -- (298.74,175.43) -- (306.53,176.32) -- (313.63,175.43) -- (321.53,171.84) -- (323.34,163.06);
\fill[E69F00] (260.42,173.23000000000002) rectangle ++(4.4pt,4.4pt);
\fill[E69F00] (285.76,173.23000000000002) rectangle ++(4.4pt,4.4pt);
\fill[E69F00] (296.54,173.23000000000002) rectangle ++(4.4pt,4.4pt);
\fill[E69F00] (304.33,174.12) rectangle ++(4.4pt,4.4pt);
\fill[E69F00] (311.43,173.23000000000002) rectangle ++(4.4pt,4.4pt);
\fill[E69F00] (319.33,169.64000000000001) rectangle ++(4.4pt,4.4pt);
\fill[E69F00] (321.14,160.86) rectangle ++(4.4pt,4.4pt);
\draw[7B61A8,pcLine] (64.88,137.63) -- (107.24,139.24) -- (126.72,137.31) -- (136.11,135.37) -- (146.51,130.15) -- (147.10,126.21);
\fill[7B61A8] (64.88,140.43) -- ++(2.8pt,-4.5pt) -- ++(-5.6pt,0) -- cycle;
\fill[7B61A8] (107.24,142.04) -- ++(2.8pt,-4.5pt) -- ++(-5.6pt,0) -- cycle;
\fill[7B61A8] (126.72,140.11) -- ++(2.8pt,-4.5pt) -- ++(-5.6pt,0) -- cycle;
\fill[7B61A8] (136.11,138.17) -- ++(2.8pt,-4.5pt) -- ++(-5.6pt,0) -- cycle;
\fill[7B61A8] (146.51,132.95) -- ++(2.8pt,-4.5pt) -- ++(-5.6pt,0) -- cycle;
\fill[7B61A8] (147.10,129.01) -- ++(2.8pt,-4.5pt) -- ++(-5.6pt,0) -- cycle;
\draw[black,line width=0.5pt] (385,48) rectangle ++(315,220);
\draw[pcGrid] (424.32,48) -- (424.32,268);
\node[anchor=north,pcTick] at (424.32,44) {0.4};
\draw[pcGrid] (502.95,48) -- (502.95,268);
\node[anchor=north,pcTick] at (502.95,44) {0.5};
\draw[pcGrid] (581.58,48) -- (581.58,268);
\node[anchor=north,pcTick] at (581.58,44) {0.6};
\draw[pcGrid] (660.22,48) -- (660.22,268);
\node[anchor=north,pcTick] at (660.22,44) {0.7};
\draw[pcGrid] (385,193.65) -- (700,193.65);
\node[anchor=south,font=\small\bfseries] at (542.5,277) {HotpotQA};
\node[anchor=north,pcTick] at (542.5,24) {Recall@100};
\draw[D62728,pcLine] (511.36,228.80) -- (562.95,223.74) -- (609.03,221.65) -- (622.24,219.75) -- (661.63,210.22) -- (671.31,202.82) -- (682.86,191.50);
\fill[D62728] (511.36,228.80) circle (2.2pt);
\fill[D62728] (562.95,223.74) circle (2.2pt);
\fill[D62728] (609.03,221.65) circle (2.2pt);
\fill[D62728] (622.24,219.75) circle (2.2pt);
\fill[D62728] (661.63,210.22) circle (2.2pt);
\fill[D62728] (671.31,202.82) circle (2.2pt);
\fill[D62728] (682.86,191.50) circle (2.2pt);
\draw[E69F00,pcLine] (554.14,215.14) -- (594.72,213.73) -- (615.95,206.66) -- (672.56,172.74) -- (676.34,162.83);
\fill[E69F00] (551.9399999999999,212.94) rectangle ++(4.4pt,4.4pt);
\fill[E69F00] (592.52,211.53) rectangle ++(4.4pt,4.4pt);
\fill[E69F00] (613.75,204.46) rectangle ++(4.4pt,4.4pt);
\fill[E69F00] (670.3599999999999,170.54000000000002) rectangle ++(4.4pt,4.4pt);
\fill[E69F00] (674.14,160.63000000000002) rectangle ++(4.4pt,4.4pt);
\draw[7B61A8,pcLine] (397.27,173.38) -- (409.85,152.63) -- (426.13,87.20);
\fill[7B61A8] (397.27,176.18) -- ++(2.8pt,-4.5pt) -- ++(-5.6pt,0) -- cycle;
\fill[7B61A8] (409.85,155.43) -- ++(2.8pt,-4.5pt) -- ++(-5.6pt,0) -- cycle;
\fill[7B61A8] (426.13,90.00) -- ++(2.8pt,-4.5pt) -- ++(-5.6pt,0) -- cycle;
\fill[D62728] (220,342) circle (2pt);
\node[anchor=west,font=\Large] at (228,337) {SIMQ(HNSW)};
\fill[E69F00] (323,340) rectangle ++(4pt,4pt);
\node[anchor=west,font=\Large] at (333,337) {k-means};
\fill[7B61A8] (428,339) -- ++(5pt,0) -- ++(-2.5pt,4pt) -- cycle;
\node[anchor=west,font=\Large] at (438,337) {LSH};
\end{tikzpicture}


==> figures/qps_recall_main.tex <==
\begin{tabular}{@{}ccccc@{}}
\multicolumn{5}{c}{%
\begin{tikzpicture}[x=1pt,y=1pt,baseline=(current bounding box.north)]
\definecolor{D62728}{HTML}{D62728}
\definecolor{9467BD}{HTML}{9467BD}
\definecolor{1F77B4}{HTML}{1F77B4}
\definecolor{2CA02C}{HTML}{2CA02C}
\definecolor{E69F00}{HTML}{E69F00}
\tikzset{legendtext/.style={font=\large}}
\fill[D62728] (13,0) circle (2.1pt);
\node[anchor=west,legendtext] at (20,-3) {SIMQ};
\fill[9467BD] (102.9,-2.1) rectangle ++(4.2pt,4.2pt);
\node[anchor=west,legendtext] at (112,-3) {GEM};
\fill[1F77B4] (203,2.5) -- ++(2.5pt,-4.1pt) -- ++(-5pt,0) -- cycle;
\node[anchor=west,legendtext] at (210,-3) {MUVERA};
\fill[2CA02C] (305,2.5) -- ++(2.5pt,-2.5pt) -- ++(-2.5pt,-2.5pt) -- ++(-2.5pt,2.5pt) -- cycle;
\node[anchor=west,legendtext] at (312,-3) {PLAID};
\draw[E69F00,line width=0.85pt] (410.5,-2.5) -- (415.5,2.5) (410.5,2.5) -- (415.5,-2.5);
\node[anchor=west,legendtext] at (420,-3) {IGP};
\end{tikzpicture}} \\[0.5ex]
\input{../figures/qps_recall_main_panels/quora_R20_20.tex} & \input{../figures/qps_recall_main_panels/scidocs_R20_20.tex} & \input{../figures/qps_recall_main_panels/lotte_beir_R20_20.tex} & \input{../figures/qps_recall_main_panels/nq_R20_20.tex} & \input{../figures/qps_recall_main_panels/hotpotqa_R20_20.tex} \\[-2ex]
\input{../figures/qps_recall_main_panels/quora_R50_50.tex} & \input{../figures/qps_recall_main_panels/scidocs_R50_50.tex} & \input{../figures/qps_recall_main_panels/lotte_beir_R50_50.tex} & \input{../figures/qps_recall_main_panels/nq_R50_50.tex} & \input{../figures/qps_recall_main_panels/hotpotqa_R50_50.tex} \\[-2ex]
\input{../figures/qps_recall_main_panels/quora_R100_100.tex} & \input{../figures/qps_recall_main_panels/scidocs_R100_100.tex} & \input{../figures/qps_recall_main_panels/lotte_beir_R100_100.tex} & \input{../figures/qps_recall_main_panels/nq_R100_100.tex} & \input{../figures/qps_recall_main_panels/hotpotqa_R100_100.tex} \\[-1ex]
\end{tabular}


==> figures/simq_alpha_sensitivity.tex <==
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{D62728}{HTML}{D62728}
\definecolor{1F77B4}{HTML}{1F77B4}
\definecolor{2CA02C}{HTML}{2CA02C}
\definecolor{9467BD}{HTML}{9467BD}
\definecolor{E69F00}{HTML}{E69F00}
\tikzset{alphaLine/.style={line width=1.45pt,line cap=round,line join=round}, alphaGrid/.style={gray!55,dashed,line width=0.25pt}, alphaTick/.style={font=\scriptsize}}
\draw[black,line width=0.4pt] (25,34) rectangle (123,91);
\draw[alphaGrid] (25.00,34) -- (25.00,91);
\node[anchor=north,alphaTick] at (25.00,32) {0.70};
\draw[alphaGrid] (49.50,34) -- (49.50,91);
\node[anchor=north,alphaTick] at (49.50,32) {0.75};
\draw[alphaGrid] (74.00,34) -- (74.00,91);
\node[anchor=north,alphaTick] at (74.00,32) {0.80};
\draw[alphaGrid] (98.50,34) -- (98.50,91);
\node[anchor=north,alphaTick] at (98.50,32) {0.85};
\draw[alphaGrid] (123.00,34) -- (123.00,91);
\node[anchor=north,alphaTick] at (123.00,32) {0.90};
\draw[alphaGrid] (25,34.00) -- (123,34.00);
\node[anchor=east,alphaTick] at (23,34.00) {100};
\draw[alphaGrid] (25,62.50) -- (123,62.50);
\node[anchor=east,alphaTick] at (23,62.50) {200};
\draw[alphaGrid] (25,91.00) -- (123,91.00);
\node[anchor=east,alphaTick] at (23,91.00) {300};
\node[rotate=90,anchor=south,alphaTick] at (13,62.5) {QPS};
\node[anchor=north,font=\scriptsize] at (74.0,24) {Recall100@100};
\draw[1F77B4,alphaLine] (39.60,55.89) -- (51.31,55.06) -- (74.54,54.49) -- (104.92,54.75) -- (111.88,52.53);
\fill[1F77B4] (39.60,55.89) circle (2.1pt);
\fill[1F77B4] (51.31,55.06) circle (2.1pt);
\fill[1F77B4] (74.54,54.49) circle (2.1pt);
\fill[1F77B4] (104.92,54.75) circle (2.1pt);
\fill[1F77B4] (111.88,52.53) circle (2.1pt);
\draw[2CA02C,alphaLine] (42.20,59.19) -- (67.63,58.48) -- (80.27,57.66) -- (105.95,56.97) -- (115.40,55.63) -- (115.80,55.55);
\fill[2CA02C] (40.40,57.39) rectangle ++(3.6pt,3.6pt);
\fill[2CA02C] (65.83,56.68) rectangle ++(3.6pt,3.6pt);
\fill[2CA02C] (78.47,55.86) rectangle ++(3.6pt,3.6pt);
\fill[2CA02C] (104.15,55.17) rectangle ++(3.6pt,3.6pt);
\fill[2CA02C] (113.60,53.83) rectangle ++(3.6pt,3.6pt);
\fill[2CA02C] (114.00,53.75) rectangle ++(3.6pt,3.6pt);
\draw[D62728,alphaLine] (38.77,59.62) -- (63.56,58.97) -- (77.48,58.65) -- (85.96,58.40) -- (91.89,57.83) -- (100.02,57.40) -- (107.08,57.37) -- (116.29,56.32);
\fill[D62728] (38.77,61.72) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (63.56,61.07) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (77.48,60.75) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (85.96,60.50) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (91.89,59.93) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (100.02,59.50) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (107.08,59.47) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (116.29,58.42) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\draw[9467BD,alphaLine] (26.81,60.82) -- (57.09,59.54) -- (71.35,59.19) -- (81.69,58.88) -- (88.70,58.71) -- (103.69,58.20) -- (117.61,57.00);
\fill[9467BD] (28.91,60.82) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\fill[9467BD] (59.19,59.54) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\fill[9467BD] (73.45,59.19) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\fill[9467BD] (83.79,58.88) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\fill[9467BD] (90.80,58.71) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\fill[9467BD] (105.79,58.20) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\fill[9467BD] (119.71,57.00) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\draw[E69F00,alphaLine] (53.81,60.19) -- (66.80,59.62) -- (84.68,59.22) -- (101.29,58.62) -- (111.88,58.14) -- (118.34,57.54);
\draw[E69F00,line width=0.9pt] (51.81,58.19) -- ++(4pt,4pt) (51.81,62.19) -- ++(4pt,-4pt);
\draw[E69F00,line width=0.9pt] (64.80,57.62) -- ++(4pt,4pt) (64.80,61.62) -- ++(4pt,-4pt);
\draw[E69F00,line width=0.9pt] (82.68,57.22) -- ++(4pt,4pt) (82.68,61.22) -- ++(4pt,-4pt);
\draw[E69F00,line width=0.9pt] (99.29,56.62) -- ++(4pt,4pt) (99.29,60.62) -- ++(4pt,-4pt);
\draw[E69F00,line width=0.9pt] (109.88,56.14) -- ++(4pt,4pt) (109.88,60.14) -- ++(4pt,-4pt);
\draw[E69F00,line width=0.9pt] (116.34,55.54) -- ++(4pt,4pt) (116.34,59.54) -- ++(4pt,-4pt);
\draw[black,line width=0.4pt] (155,34) rectangle (253,91);
\draw[alphaGrid] (164.80,34) -- (164.80,91);
\node[anchor=north,alphaTick] at (164.80,32) {0.80};
\draw[alphaGrid] (189.30,34) -- (189.30,91);
\node[anchor=north,alphaTick] at (189.30,32) {0.85};
\draw[alphaGrid] (213.80,34) -- (213.80,91);
\node[anchor=north,alphaTick] at (213.80,32) {0.90};
\draw[alphaGrid] (238.30,34) -- (238.30,91);
\node[anchor=north,alphaTick] at (238.30,32) {0.95};
\draw[alphaGrid] (155,34.00) -- (253,34.00);
\node[anchor=east,alphaTick] at (153,34.00) {400};
\draw[alphaGrid] (155,53.00) -- (253,53.00);
\node[anchor=east,alphaTick] at (153,53.00) {500};
\draw[alphaGrid] (155,72.00) -- (253,72.00);
\node[anchor=east,alphaTick] at (153,72.00) {600};
\draw[alphaGrid] (155,91.00) -- (253,91.00);
\node[anchor=east,alphaTick] at (153,91.00) {700};
\node[rotate=90,anchor=south,alphaTick] at (138,62.5) {QPS};
\node[anchor=north,font=\scriptsize] at (204.0,24) {Recall100@100};
\draw[1F77B4,alphaLine] (168.52,53.08) -- (193.96,53.55) -- (203.56,53.86) -- (211.99,54.05) -- (228.40,54.16) -- (228.40,53.95);
\fill[1F77B4] (168.52,53.08) circle (2.1pt);
\fill[1F77B4] (193.96,53.55) circle (2.1pt);
\fill[1F77B4] (203.56,53.86) circle (2.1pt);
\fill[1F77B4] (211.99,54.05) circle (2.1pt);
\fill[1F77B4] (228.40,54.16) circle (2.1pt);
\fill[1F77B4] (228.40,53.95) circle (2.1pt);
\draw[2CA02C,alphaLine] (161.37,54.12) -- (186.31,54.73) -- (200.08,55.03) -- (211.40,55.20) -- (221.30,55.43) -- (233.35,54.86);
\fill[2CA02C] (159.57,52.32) rectangle ++(3.6pt,3.6pt);
\fill[2CA02C] (184.51,52.93) rectangle ++(3.6pt,3.6pt);
\fill[2CA02C] (198.28,53.23) rectangle ++(3.6pt,3.6pt);
\fill[2CA02C] (209.60,53.40) rectangle ++(3.6pt,3.6pt);
\fill[2CA02C] (219.50,53.63) rectangle ++(3.6pt,3.6pt);
\fill[2CA02C] (231.55,53.06) rectangle ++(3.6pt,3.6pt);
\draw[D62728,alphaLine] (159.85,62.18) -- (171.17,59.23) -- (181.41,59.21) -- (196.50,59.54) -- (208.16,59.78) -- (221.39,60.28);
\fill[D62728] (159.85,64.28) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (171.17,61.33) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (181.41,61.31) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (196.50,61.64) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (208.16,61.88) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[D62728] (221.39,62.38) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\draw[9467BD,alphaLine] (175.09,53.84) -- (188.27,53.63) -- (206.11,54.12) -- (220.90,54.35) -- (230.46,54.54) -- (241.19,55.00);
\fill[9467BD] (177.19,53.84) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\fill[9467BD] (190.37,53.63) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\fill[9467BD] (208.21,54.12) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\fill[9467BD] (223.00,54.35) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\fill[9467BD] (232.56,54.54) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\fill[9467BD] (243.29,55.00) -- ++(-2.1pt,2.1pt) -- ++(-2.1pt,-2.1pt) -- ++(2.1pt,-2.1pt) -- cycle;
\draw[E69F00,alphaLine] (183.76,55.03) -- (201.16,55.19) -- (215.32,55.47) -- (230.90,55.91) -- (244.33,55.34);
\draw[E69F00,line width=0.9pt] (181.76,53.03) -- ++(4pt,4pt) (181.76,57.03) -- ++(4pt,-4pt);
\draw[E69F00,line width=0.9pt] (199.16,53.19) -- ++(4pt,4pt) (199.16,57.19) -- ++(4pt,-4pt);
\draw[E69F00,line width=0.9pt] (213.32,53.47) -- ++(4pt,4pt) (213.32,57.47) -- ++(4pt,-4pt);
\draw[E69F00,line width=0.9pt] (228.90,53.91) -- ++(4pt,4pt) (228.90,57.91) -- ++(4pt,-4pt);
\draw[E69F00,line width=0.9pt] (242.33,53.34) -- ++(4pt,4pt) (242.33,57.34) -- ++(4pt,-4pt);
\draw[1F77B4,alphaLine] (23,12) -- (30,12);
\fill[1F77B4] (26.5,12) circle (2pt);
\node[anchor=west,font=\scriptsize] at (32,12) {$\alpha=0.05$};
\draw[2CA02C,alphaLine] (101,12) -- (108,12);
\fill[2CA02C] (102.7,10.2) rectangle ++(3.6pt,3.6pt);
\node[anchor=west,font=\scriptsize] at (110,12) {$\alpha=0.08$};
\draw[D62728,alphaLine] (179,12) -- (186,12);
\fill[D62728] (182.5,14) -- ++(2.5pt,-4pt) -- ++(-5pt,0) -- cycle;
\node[anchor=west,font=\scriptsize] at (188,12) {$\alpha=0.1$ (default)};
\draw[9467BD,alphaLine] (62,2) -- (69,2);
\fill[9467BD] (65.5,4) -- ++(2pt,-2pt) -- ++(-2pt,-2pt) -- ++(-2pt,2pt) -- cycle;
\node[anchor=west,font=\scriptsize] at (71,2) {$\alpha=0.15$};
\draw[E69F00,alphaLine] (158,2) -- (165,2);
\draw[E69F00,line width=0.9pt] (159.5,0) -- ++(4pt,4pt) (159.5,4) -- ++(4pt,-4pt);
\node[anchor=west,font=\scriptsize] at (167,2) {$\alpha=0.20$};
\end{tikzpicture}


==> figures/simq_simqplus_m_recall.tex <==
\begin{tikzpicture}[x=1pt,y=1pt,baseline=(current bounding box.north)]
\definecolor{D62728}{HTML}{D62728}
\definecolor{1F77B4}{HTML}{1F77B4}
\fill[D62728] (10,5) circle (2.1pt);
\node[anchor=west,font=\scriptsize] at (16,5) {SIMQ};
\fill[1F77B4] (80,7.3) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\node[anchor=west,font=\scriptsize] at (88,5) {SIMQ+};
\end{tikzpicture}
\vspace{-1.2ex}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{@{}c@{\hspace{2pt}}c@{}}
\input{../figures/simq_simqplus_m_recall_panels/lotte_beir.tex} & \input{../figures/simq_simqplus_m_recall_panels/nq.tex} \\[-1.5ex]
\input{../figures/simq_simqplus_m_recall_panels/hotpotqa.tex} & \input{../figures/simq_simqplus_m_recall_panels/quora.tex}
\end{tabular}


==> figures/simq_simqplus_m_recall_panels/hotpotqa.tex <==
\begin{tikzpicture}[x=1pt,y=1pt,baseline=(current bounding box.north)]
\definecolor{D62728}{HTML}{D62728}
\definecolor{1F77B4}{HTML}{1F77B4}
\tikzset{panelLine/.style={line width=1.45pt,line cap=round,line join=round}, panelGrid/.style={gray!55,dashed,line width=0.25pt}, panelTick/.style={font=\scriptsize}}
\draw[black,line width=0.4pt] (32.00,20.00) rectangle ++(85.00,70.00);
\draw[panelGrid] (32.00,20.00) -- (32.00,90.00);
\node[anchor=north,panelTick] at (32.00,18.00) {10};
\draw[panelGrid] (68.94,20.00) -- (68.94,90.00);
\node[anchor=north,panelTick] at (68.94,18.00) {100};
\draw[panelGrid] (105.88,20.00) -- (105.88,90.00);
\node[anchor=north,panelTick] at (105.88,18.00) {1000};
\draw[panelGrid] (32.00,20.00) -- (117.00,20.00);
\node[anchor=east,panelTick] at (30.00,21.50) {0.2};
\draw[panelGrid] (32.00,37.50) -- (117.00,37.50);
\node[anchor=east,panelTick] at (30.00,39.00) {0.4};
\draw[panelGrid] (32.00,55.00) -- (117.00,55.00);
\node[anchor=east,panelTick] at (30.00,56.50) {0.6};
\draw[panelGrid] (32.00,72.50) -- (117.00,72.50);
\node[anchor=east,panelTick] at (30.00,74.00) {0.8};
\draw[panelGrid] (32.00,90.00) -- (117.00,90.00);
\node[anchor=east,panelTick] at (30.00,91.50) {1.0};
\node[anchor=north,panelTick] at (74.50,7.00) {$n_c$};
\node[rotate=90,panelTick] at (7.5,55.00) {Recall@100};
\draw[D62728,panelLine] (32.00,27.62) -- (57.82,41.68) -- (80.06,52.93) -- (91.18,58.05) -- (100.16,61.71) -- (105.88,63.91) -- (111.28,65.88) -- (117.00,67.90);
\fill[D62728] (32.00,27.62) circle (2.1pt);
\fill[D62728] (57.82,41.68) circle (2.1pt);
\fill[D62728] (80.06,52.93) circle (2.1pt);
\fill[D62728] (91.18,58.05) circle (2.1pt);
\fill[D62728] (100.16,61.71) circle (2.1pt);
\fill[D62728] (105.88,63.91) circle (2.1pt);
\fill[D62728] (111.28,65.88) circle (2.1pt);
\fill[D62728] (117.00,67.90) circle (2.1pt);
\draw[1F77B4,panelLine] (32.00,35.36) -- (57.82,45.37) -- (80.06,57.80) -- (91.18,62.38) -- (100.16,65.69) -- (105.88,67.53) -- (111.28,69.29) -- (117.00,70.97);
\fill[1F77B4] (32.00,37.66) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (57.82,47.67) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (80.06,60.10) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (91.18,64.69) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (100.16,67.99) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (105.88,69.83) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (111.28,71.59) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (117.00,73.27) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\end{tikzpicture}


==> figures/simq_simqplus_m_recall_panels/lotte_beir.tex <==
\begin{tikzpicture}[x=1pt,y=1pt,baseline=(current bounding box.north)]
\definecolor{D62728}{HTML}{D62728}
\definecolor{1F77B4}{HTML}{1F77B4}
\tikzset{panelLine/.style={line width=1.45pt,line cap=round,line join=round}, panelGrid/.style={gray!55,dashed,line width=0.25pt}, panelTick/.style={font=\scriptsize}}
\draw[black,line width=0.4pt] (32.00,20.00) rectangle ++(85.00,70.00);
\draw[panelGrid] (32.00,20.00) -- (32.00,90.00);
\node[anchor=north,panelTick] at (32.00,18.00) {10};
\draw[panelGrid] (68.94,20.00) -- (68.94,90.00);
\node[anchor=north,panelTick] at (68.94,18.00) {100};
\draw[panelGrid] (105.88,20.00) -- (105.88,90.00);
\node[anchor=north,panelTick] at (105.88,18.00) {1000};
\draw[panelGrid] (32.00,20.00) -- (117.00,20.00);
\node[anchor=east,panelTick] at (30.00,21.50) {0.2};
\draw[panelGrid] (32.00,37.50) -- (117.00,37.50);
\node[anchor=east,panelTick] at (30.00,39.00) {0.4};
\draw[panelGrid] (32.00,55.00) -- (117.00,55.00);
\node[anchor=east,panelTick] at (30.00,56.50) {0.6};
\draw[panelGrid] (32.00,72.50) -- (117.00,72.50);
\node[anchor=east,panelTick] at (30.00,74.00) {0.8};
\draw[panelGrid] (32.00,90.00) -- (117.00,90.00);
\node[anchor=east,panelTick] at (30.00,91.50) {1.0};
\node[anchor=north,panelTick] at (74.50,7.00) {$n_c$};
\node[rotate=90,panelTick] at (7.5,55.00) {Recall@100};
\draw[D62728,panelLine] (32.00,41.72) -- (57.82,52.88) -- (68.94,59.10) -- (86.56,67.41) -- (97.68,71.50) -- (104.19,73.31) -- (108.80,74.42) -- (113.42,75.47) -- (117.00,76.06);
\fill[D62728] (32.00,41.72) circle (2.1pt);
\fill[D62728] (57.82,52.88) circle (2.1pt);
\fill[D62728] (68.94,59.10) circle (2.1pt);
\fill[D62728] (86.56,67.41) circle (2.1pt);
\fill[D62728] (97.68,71.50) circle (2.1pt);
\fill[D62728] (104.19,73.31) circle (2.1pt);
\fill[D62728] (108.80,74.42) circle (2.1pt);
\fill[D62728] (113.42,75.47) circle (2.1pt);
\fill[D62728] (117.00,76.06) circle (2.1pt);
\draw[1F77B4,panelLine] (32.00,44.26) -- (57.82,56.50) -- (68.94,62.78) -- (86.56,71.13) -- (97.68,74.11) -- (104.19,75.75) -- (108.80,76.60) -- (113.42,77.30) -- (117.00,77.60);
\fill[1F77B4] (32.00,46.56) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (57.82,58.80) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (68.94,65.08) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (86.56,73.43) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (97.68,76.41) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (104.19,78.05) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (108.80,78.90) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (113.42,79.60) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (117.00,79.90) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\end{tikzpicture}


==> figures/simq_simqplus_m_recall_panels/nq.tex <==
\begin{tikzpicture}[x=1pt,y=1pt,baseline=(current bounding box.north)]
\definecolor{D62728}{HTML}{D62728}
\definecolor{1F77B4}{HTML}{1F77B4}
\tikzset{panelLine/.style={line width=1.45pt,line cap=round,line join=round}, panelGrid/.style={gray!55,dashed,line width=0.25pt}, panelTick/.style={font=\scriptsize}}
\draw[black,line width=0.4pt] (32.00,20.00) rectangle ++(85.00,70.00);
\draw[panelGrid] (32.00,20.00) -- (32.00,90.00);
\node[anchor=north,panelTick] at (32.00,18.00) {10};
\draw[panelGrid] (68.94,20.00) -- (68.94,90.00);
\node[anchor=north,panelTick] at (68.94,18.00) {100};
\draw[panelGrid] (105.88,20.00) -- (105.88,90.00);
\node[anchor=north,panelTick] at (105.88,18.00) {1000};
\draw[panelGrid] (32.00,20.00) -- (117.00,20.00);
\node[anchor=east,panelTick] at (30.00,21.50) {0.2};
\draw[panelGrid] (32.00,37.50) -- (117.00,37.50);
\node[anchor=east,panelTick] at (30.00,39.00) {0.4};
\draw[panelGrid] (32.00,55.00) -- (117.00,55.00);
\node[anchor=east,panelTick] at (30.00,56.50) {0.6};
\draw[panelGrid] (32.00,72.50) -- (117.00,72.50);
\node[anchor=east,panelTick] at (30.00,74.00) {0.8};
\draw[panelGrid] (32.00,90.00) -- (117.00,90.00);
\node[anchor=east,panelTick] at (30.00,91.50) {1.0};
\node[anchor=north,panelTick] at (74.50,7.00) {$n_c$};
\node[rotate=90,panelTick] at (7.5,55.00) {Recall@100};
\draw[D62728,panelLine] (32.00,47.83) -- (57.82,60.00) -- (68.94,66.21) -- (91.18,74.64) -- (97.68,76.53) -- (104.19,78.00) -- (108.80,78.91) -- (113.42,79.54) -- (117.00,80.05);
\fill[D62728] (32.00,47.83) circle (2.1pt);
\fill[D62728] (57.82,60.00) circle (2.1pt);
\fill[D62728] (68.94,66.21) circle (2.1pt);
\fill[D62728] (91.18,74.64) circle (2.1pt);
\fill[D62728] (97.68,76.53) circle (2.1pt);
\fill[D62728] (104.19,78.00) circle (2.1pt);
\fill[D62728] (108.80,78.91) circle (2.1pt);
\fill[D62728] (113.42,79.54) circle (2.1pt);
\fill[D62728] (117.00,80.05) circle (2.1pt);
\draw[1F77B4,panelLine] (32.00,50.76) -- (57.82,63.47) -- (68.94,69.82) -- (91.18,77.79) -- (97.68,79.40) -- (104.19,80.40) -- (108.80,80.90) -- (113.42,81.39) -- (117.00,81.55);
\fill[1F77B4] (32.00,53.06) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (57.82,65.77) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (68.94,72.12) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (91.18,80.09) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (97.68,81.70) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (104.19,82.70) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (108.80,83.20) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (113.42,83.69) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (117.00,83.85) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\end{tikzpicture}


==> figures/simq_simqplus_m_recall_panels/quora.tex <==
\begin{tikzpicture}[x=1pt,y=1pt,baseline=(current bounding box.north)]
\definecolor{D62728}{HTML}{D62728}
\definecolor{1F77B4}{HTML}{1F77B4}
\tikzset{panelLine/.style={line width=1.45pt,line cap=round,line join=round}, panelGrid/.style={gray!55,dashed,line width=0.25pt}, panelTick/.style={font=\scriptsize}}
\draw[black,line width=0.4pt] (32.00,20.00) rectangle ++(85.00,70.00);
\draw[panelGrid] (32.00,20.00) -- (32.00,90.00);
\node[anchor=north,panelTick] at (32.00,18.00) {2};
\draw[panelGrid] (66.97,20.00) -- (66.97,90.00);
\node[anchor=north,panelTick] at (66.97,18.00) {10};
\draw[panelGrid] (101.94,20.00) -- (101.94,90.00);
\node[anchor=north,panelTick] at (101.94,18.00) {50};
\draw[panelGrid] (117.00,20.00) -- (117.00,90.00);
\node[anchor=north,panelTick] at (117.00,18.00) {100};
\draw[panelGrid] (32.00,20.00) -- (117.00,20.00);
\node[anchor=east,panelTick] at (30.00,21.50) {0.2};
\draw[panelGrid] (32.00,37.50) -- (117.00,37.50);
\node[anchor=east,panelTick] at (30.00,39.00) {0.4};
\draw[panelGrid] (32.00,55.00) -- (117.00,55.00);
\node[anchor=east,panelTick] at (30.00,56.50) {0.6};
\draw[panelGrid] (32.00,72.50) -- (117.00,72.50);
\node[anchor=east,panelTick] at (30.00,74.00) {0.8};
\draw[panelGrid] (32.00,90.00) -- (117.00,90.00);
\node[anchor=east,panelTick] at (30.00,91.50) {1.0};
\node[anchor=north,panelTick] at (74.50,7.00) {$n_c$};
\node[rotate=90,panelTick] at (7.5,55.00) {Recall@100};
\draw[D62728,panelLine] (32.00,48.00) -- (51.91,64.80) -- (86.88,77.01) -- (99.65,80.24) -- (105.90,81.24) -- (112.15,82.09) -- (117.00,82.61);
\fill[D62728] (32.00,48.00) circle (2.1pt);
\fill[D62728] (51.91,64.80) circle (2.1pt);
\fill[D62728] (86.88,77.01) circle (2.1pt);
\fill[D62728] (99.65,80.24) circle (2.1pt);
\fill[D62728] (105.90,81.24) circle (2.1pt);
\fill[D62728] (112.15,82.09) circle (2.1pt);
\fill[D62728] (117.00,82.61) circle (2.1pt);
\draw[1F77B4,panelLine] (32.00,48.00) -- (51.91,65.16) -- (86.88,79.84) -- (99.65,81.91) -- (105.90,83.27) -- (112.15,84.25) -- (117.00,84.65);
\fill[1F77B4] (32.00,50.30) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (51.91,67.46) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (86.88,82.14) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (99.65,84.21) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (105.90,85.57) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (112.15,86.55) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\fill[1F77B4] (117.00,86.95) -- ++(2.5pt,-4.2pt) -- ++(-5pt,0) -- cycle;
\end{tikzpicture}

